CM2: Reinforcement Learning with Checklist Rewards for Multi-Turn and Multi-Step Agentic Tool Use

AI agents are increasingly used to solve real-world tasks by reasoning over multi-turn user interactions and invoking external tools. However, applying reinforcement learning to such settings remains difficult: realistic objectives often lack verifiable rewards and instead emphasize open-ended behaviors; moreover, RL for multi-turn, multi-step agentic tool use is still underexplored; and building and maintaining executable tool environments is costly, limiting scale and coverage. We propose CM2, an RL framework that replaces verifiable outcome rewards with checklist rewards. CM2 decomposes each turn's intended behavior into fine-grained binary criteria with explicit evidence grounding and structured metadata, turning open-ended judging into more stable classification-style decisions. To balance stability and informativeness, our method adopts a strategy of sparse reward assignment but dense evaluation criteria. Training is performed in a scalable LLM-simulated tool environment, avoiding heavy engineering for large tool sets. Experiments show that CM2 consistently improves over supervised fine-tuning. Starting from an 8B Base model and training on an 8k-example RL dataset, CM2 improves over the SFT counterpart by 8 points on tau^-Bench, by 10 points on BFCL-V4, and by 12 points on ToolSandbox. The results match or even outperform similarly sized open-source baselines, including the judging model. CM2 thus provides a scalable recipe for optimizing multi-turn, multi-step tool-using agents without relying on verifiable rewards. Code provided by the open-source community: https://github.com/namezhenzhang/CM2-RLCR-Tool-Agent.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec_arxiv/5_results.tex <==



% --- 第一组图：训练集指标 ---
% \begin{figure}[htbp] % 建议使用 htbp 让 LaTeX 自动寻找最佳位置
%     \centering
%     % 第一张子图
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering % 子图内部居中
%         \includegraphics[width=\textwidth]{fig/reward_norm_train.pdf}
%         \caption{Normalized Reward} % 术语稍微正式一点
%         \label{fig:reward_norm_train}
%     \end{subfigure}
%     \hfill % <--- 关键：加上这个让三张图均匀分布
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/num_turns_train.pdf}
%         \caption{Average Turns}
%         \label{fig:num_turns_train}
%     \end{subfigure}
%     \hfill % <--- 关键
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/response_length_train.pdf}
%         \caption{Response Length}
%         \label{fig:response_length_train}
%     \end{subfigure}
    
%     % 主标题：概括这三张图是在展示训练过程的动态
%     \caption{\textbf{Training dynamics.} Evolution of the normalized reward, average number of turns, and response length during the training phase.}
%     \label{fig:metrics_train}
% \end{figure}


% --- 第二组图：验证集指标 ---
% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/reward_norm_val.pdf}
%         % 修正：原代码这里文件名是 reward，caption 却是 length，已修正
%         \caption{Normalized Reward (Val)} 
%         \label{fig:reward_norm_val} % 修正：原代码 label 重复，改为 _val
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/num_turns_val.pdf}
%         \caption{Average Turns (Val)}
%         \label{fig:num_turns_val} % 修正：原代码 label 重复，改为 _val
%     \end{subfigure}
    
%     % 主标题
%     \caption{\textbf{Validation metrics.} Performance evaluation on the validation set in terms of reward and conversation turns.}
%     \label{fig:metrics_val}
% \end{figure}

\section{Results}

% 导言区加：

\begin{figure*}[!t]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/compare_reward_level.pdf}
    \caption{Reward curves on the validation set for different advantage assignment granularities.}
    \label{fig:allocation_comparison}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/compare_n.pdf}
    \caption{Reward curves on the validation set between different group sizes ($n$).}
    \label{fig:group_size_comparison}
  \end{subfigure}

  \caption{Comparison results under different settings.}
  \label{fig:two_in_one}
\end{figure*}



\subsection{Effect of Allocation Granularity}
Figure~\ref{fig:allocation_comparison} compares the reward curve on validation set under different assignment granularities. Finer-grained allocation yields faster early improvements: step-level advantages outperform turn-level, which in turn outperform trajectory-level in the initial phase.
As training continues, however, finer granularities exhibit earlier and more severe training collapse, while trajectory-level advantages remain more stable and continue to improve. 

\noindent We attribute this trade-off to noise amplification in agentic RL. Checklist rewards reduce judge variance by turning open-ended scoring into binary, evidence-grounded decisions, but they do not eliminate stochasticity. With finer-grained assignment, this residual noise enters optimization more frequently and can be amplified by group-relative normalization, yielding higher-variance or sometimes misleading gradients. This motivates our principle of \emph{Sparse in assignment; Dense in criteria}: we keep evaluation criteria fine-grained for informative supervision, while assigning rewards at coarser granularity to average out residual noise and improve stability.


\subsection{Effect of Group Size}
Figure~\ref{fig:group_size_comparison} shows the impact of group size $G$ (e.g., $G{=}24$ vs.\ $G{=}48$) with trajectory-level Checklist rewards. A larger group size consistently achieves higher rewards. Intuitively, for multi-turn, multi-step trajectories, increasing $G$ provides more samples for later turns, leading to a lower-variance advantage estimate more reliable gradient updates.

% \subsection{Training Dynamics}
% Additional training dynamics are reported in Appendix~\ref{app:training_dynamics}.



% 我们在图 2 中展示了使用不同 allocation 细粒度的 advantage，rl 训练过程中在 validation set 上的 reward 变化曲线。我们可以看到，越细粒度的 advantage，在初期增长的越快（橙色 step level 大于蓝色 turn level 大于绿色 trajectory level）。但随着步数增多，越细粒度的 advantage，训练奔溃得越快，而只有 trajectory level 的一直在稳定增长。我们认为这是由于 rl 的训练过程中存在着一定的噪音。虽然细粒度的 advantage 提供了更细致的监督信号，但由于存在噪声，可能提供错误的监督信号。而粗粒度的信号对于错误更加鲁棒。

% 我们在图 3 中 展示了不同的group 大小（n=24 and 48）的 reward 曲线。我们可以发现更大的 n （48）可以获得更高的 reward。

% 更多的训练细节和 training dynamic 请见 appendix.

% We present the 

% We present the training dynamics in Figure \ref{fig:metrics_train}. As shown in Figure \ref{fig:metrics_train}(a), the normalized reward steadily increases and converges, demonstrating the effectiveness of our optimization process. Interestingly, we observe a concurrent upward trend in both the average number of turns (Figure \ref{fig:metrics_train}(b)) and the response length (Figure \ref{fig:metrics_train}(c)). This suggests that the model learns to sustain longer interactions and generate more comprehensive responses to maximize the reward signal.

% To verify the robustness of our approach, we further evaluate the model on the validation set. Figure \ref{fig:metrics_val} illustrates the evolution of the normalized reward and average turns during validation. The consistent improvement in validation metrics aligns with the training curves, indicating that our model generalizes well to unseen data without suffering from severe overfitting.


\subsection{Results on Benchmarks}

% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Model / Method} & \textbf{airline} & \textbf{retail} & \textbf{telecom} & \textbf{mock} & \textbf{Avg.} \\
% \midrule
% \rowcolor{gray!12}
% \multicolumn{6}{l}{\textit{Open-source models}} \\
% Qwen3-30B-A3B-Instruct-2507 & 32.50 & 50.88 & 12.72 & 88.89 & 46.25 \\
% Qwen3-8B-Thinking & 30.00 & 43.64 & 22.37 & 86.11 & 45.53 \\
% \rowcolor{gray!12}
% \multicolumn{6}{l}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
% \quad Cold-start SFT on $\mathcal{D}_{\text{CS}}$ & 25.50 & 18.42 & 11.84 & 77.78 & 33.39 \\
% \quad\quad $\hookrightarrow$ SFT on $\mathcal{D}_{\text{RL}}$ & 23.50 & 19.52 & 12.06 & 72.22 & 31.83\\
% \quad\quad $\hookrightarrow$ RL on $\mathcal{D}_{\text{RL}}$ (\method) & 27.00 & 36.40 & 16.89 & 80.56 & 40.21 \\
% \bottomrule
% \end{tabular}}
% \caption{Results on the $\tau^2$-Bench benchmark.

\setlength{\tabcolsep}{4pt}
\begin{table}[!t]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Model / Method} & \textbf{Airline} & \textbf{Retail} & \textbf{Telecom} & \textbf{Avg.} \\
\midrule
\rowcolor{gray!12}
\multicolumn{5}{c}{\textit{Open-source Baselines}} \\
Qwen3-30B-A3B-Instruct-2507 & 32.50 & 50.88 & 12.72 & 32.03 \\
Qwen3-8B-Thinking & 30.00 & 43.64 & 22.37 & 32.00 \\
\rowcolor{gray!12}
\multicolumn{5}{c}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
Cold-start SFT on $\mathcal{D}_{\text{CS}}$ & 25.50 & 18.42 & 11.84 & 18.59 \\
\quad $\hookrightarrow$ SFT on $\mathcal{D}_{\text{RL}}$ & 23.50 & 19.52 & 12.06 & 18.36 \\
\quad $\hookrightarrow$ RL on $\mathcal{D}_{\text{RL}}$ (\method) & 27.00 & 36.40 & 16.89 & 26.76 \\
\rowcolor{gray!12}
\multicolumn{5}{l}{\textit{Ours} (from \textbf{Qwen3-8B-Thinking})} \\
\quad SFT on $\mathcal{D}_{\text{APIGen}}$ & 30.00& 44.74 & 23.68 & 32.81 \\
\quad RL on $\mathcal{D}_{\text{APIGen}}$ (\method-$\tau^2$) & 33.00 & 54.17 & 37.00 & 41.39 \\
\bottomrule
\end{tabular}}
\caption{Results on the $\tau^2$-Bench benchmark. We run evaluation four times and report the average accuracy
We follow the default evaluation setting of $\tau^2$-Bench, except that we retain the thinking content for our models to align with our training setup.
We further conduct SFT and RL with apigen-mt-5k \cite{prabhakar2025apigen}, a sythetic dataset for $\tau$-Bench. It shares the same tool functions on airline and retail subset while telecom is not covered.
}
\label{tab:tau2_bench}
\end{table}


% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model / Method} & \textbf{airline} & \textbf{retail} & \textbf{telecom} & \textbf{\sout{Avg.}} \\
% \midrule
% \rowcolor{gray!12}
% \multicolumn{5}{l}{\textit{Open-source models}} \\
% %Qwen3-8B-Thinking & 30.00 & 43.64 & 22.37 & \sout{} \\
% %Qwen3-8B-Thinking2 & 34.00 & 33.92 &  & \sout{} \\
% Qwen3-8B-keepthink & 35.33 & 36.26  & 19.59 & \sout{} \\
% % Qwen3-8B-NoThinking & 15.53 & 33.92 & 21.07 & \sout{} \\
% Qwen3-8B + SFT  & 31.33 & 41.52 & 22.81 & \sout{} \\
% Qwen3-8B + RL & 34.67 & 44.15  &  25.15 & \sout{xx} \\
% % Qwen3-8B + RL-mixed & 37.33 & 50.58  & 32.75 & \sout{xx} \\
% % Qwen3-8B + RL-mixed-2 & 35.33 & 52.92  & 37.43 & \sout{xx} \\
% \bottomrule
% \end{tabular}}
% \caption{Results on the $\tau^2$-Bench benchmark. We conduct SFT and RL with apigen-mt-5k \cite{prabhakar2025apigen} .apigen-mt-5k is sythensized dataset for tau-bench. and thus it shares the same tool functions on airline and retail as $\tau^2$-bench while telecom is not included in the training.}
% \label{tab:tau2_sft_vs_rl}
% \end{table}

\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cccccccc}
\toprule
& \multicolumn{5}{c}{\textbf{Multi-Turn}} & \multicolumn{3}{c}{\textbf{Web Search}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-9}
\textbf{Model / Method}  & \textbf{Base} & \textbf{Miss Func} & \textbf{Miss Param} & \textbf{Long Ctx} & \textbf{Overall} & \textbf{Base} & \textbf{No Snippet} & \textbf{Overall} \\
\midrule
\rowcolor{gray!12}
\multicolumn{9}{c}{\textit{Open-source Baselines}} \\
Qwen3-30B-A3B-Instruct-2507  & 45.0 & 28.0 & 21.0 & 42.5 & \textit{34.25}  &	24.00 &	17.00 & 20.50\\
Qwen3-8B-Thinking & 42.5 & 38.5 & 31.5 & 35.5 & \textit{37.00} & 	19.00 & 11.00 & 15.00 \\
\rowcolor{gray!12}
\multicolumn{9}{c}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
Cold-start SFT on $\mathcal{D}_{\text{CS}}$  & 24.5 & 19.0 & 14.5 & 19.5 & \textit{19.37} & 18.00 & 10.00 & 14.00 \\
\quad $\hookrightarrow$ SFT on $\mathcal{D}_{\text{RL}}$  & 30.0 & 27.5 & 24.5 & 25.0 & \textit{26.75} & 18.00 & 9.00 & 13.50 \\
\quad $\hookrightarrow$ RL on $\mathcal{D}_{\text{RL}}$ (\method) & 44.5 & 32.0 & 35.0 & 34.5 & \textit{\textbf{36.50}} & 41.00 & 14.00 & \textbf{27.50} \\
\bottomrule
\end{tabular}%
}
\caption{Results on the BFCL-V4 benchmark (Multi-Turn and Web Search subset).
% Our models are trained from \textbf{Qwen3-8B-Base}; we do not report results for the base checkpoint since it is not instruction-tuned under this evaluation protocol.
}
\label{tab:bfcl_results}
\end{table}

% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l c}
% \toprule
% \textbf{Model / Method} & \textbf{MMAU Tool Use} $\uparrow$ \\
% \midrule
% \rowcolor{gray!12}
% \multicolumn{2}{l}{\textit{Open-source baselines}} \\
% \quad Qwen3-30B-A3B-Instruct-2507 & 62.54 \\
% \quad Qwen3-8B-Thinking & 63.87 \\
% \rowcolor{gray!12}
% \multicolumn{2}{l}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
% \quad w/ SFT on $\mathcal{D}_{\text{CS}}$ & 60.91 \\
% \quad w/ SFT on $\mathcal{D}_{\text{CS}} \cup \mathcal{D}_{\text{RL}}$ & -- \\
% \quad w/ SFT on $\mathcal{D}_{\text{CS}}$ + RL on $\mathcal{D}_{\text{RL}}$ & 59.70 \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Results on the MMAU benchmark.
% Our models are trained from \textbf{Qwen3-8B-Base}; we do not report results for the base checkpoint since it is not instruction-tuned under this evaluation protocol.}
% \label{tab:mmau_results}
% \end{table}


% \begin{table}[!t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l c}
% \toprule
% \textbf{Model / Method} & \textbf{MMAU Tool Use} $\uparrow$ \\
% \midrule
% \rowcolor{gray!12}
% \multicolumn{2}{l}{\textit{Open-source baselines}} \\
% \quad Qwen3-30B-A3B-Instruct-2507 & 63.25 \\
% \quad Qwen3-8B-Thinking & 63.87 \\
% \rowcolor{gray!12}
% \multicolumn{2}{l}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
% \quad Cold-start SFT on $\mathcal{D}_{\text{CS}}$ & 61.62 \\
% \quad\quad $\hookrightarrow$ SFT on $\mathcal{D}_{\text{RL}}$ & 62.23 \\
% \quad\quad $\hookrightarrow$ RL on $\mathcal{D}_{\text{RL}}$ (\method) & 59.70 \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Results on the MMAU benchmark.
% Our models are trained from \textbf{Qwen3-8B-Base}; we do not report results for the base checkpoint since it is not instruction-tuned under this evaluation protocol.}
% \label{tab:mmau_results}
% \end{table}




% % 定义图片中的颜色
% \definecolor{bg-gray}{gray}{0.92} % 浅灰色背景
% \definecolor{bg-blue}{RGB}{160, 170, 255} % 浅紫色/蓝色高亮


\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c ccccccc cccccccc}
\toprule
\textbf{Model / Method} &
\textbf{Overall Score} $\uparrow$ &
\multicolumn{7}{c}{\textbf{Scenario Categories}} &
\multicolumn{8}{c}{\textbf{Tool Augmentations}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-9} \cmidrule(lr){10-17}
&
&
\textbf{STC} & \textbf{MTC} & \textbf{SUT} & \textbf{MUT} & \textbf{SD} & \textbf{C} & \textbf{II} &
\textbf{0-DT} & \textbf{3-DT} & \textbf{10-DT} & \textbf{AT} & \textbf{TNS} & \textbf{TDS} & \textbf{ADS} & \textbf{ATS} \\
\midrule
\rowcolor{gray!12}
\multicolumn{17}{c}{\textit{Open-source Baselines}} \\
Qwen3-30B-A3B-Instruct-2507 & 65.24 & 84.18 & 69.14 & 74.52 & 65.33 & 75.11 & 66.95 & 40.97 & 64.29 & 68.23 & 60.98 & 66.62 & 68.56 & 63.32 & 66.17 & 63.74 \\
Qwen3-8B-Thinking & 65.47 & 77.12 & 58.91 & 64.07 & 57.82 & 60.65 & 56.71 & 76.77 & 70.96 & 67.69 & 64.55 & 60.79 & 69.00 & 56.98 & 65.08 & 68.71 \\
\rowcolor{gray!12}
\multicolumn{17}{c}{\textit{Ours} (from \textbf{Qwen3-8B-Base})} \\
Cold-start SFT on $\mathcal{D}_{\text{CS}}$ & 56.19 & 71.65 & 47.89 & 54.91 & 45.72 & 63.08 & 45.93 & 69.97 & 55.44 & 56.68 & 56.03 & 53.86 & 60.34 & 55.81 & 52.82 & 58.53 \\
\quad $\hookrightarrow$ SFT on $\mathcal{D}_{\text{RL}}$ & 55.32 & 74.89 & 46.66 & 55.71 & 42.22 & 59.25 & 44.35 & 67.41 & 55.69 & 54.09 & 55.23 & 50.42 & 62.42 & 55.27 & 53.42 & 56.04 \\
\quad $\hookrightarrow$ RL on $\mathcal{D}_{\text{RL}}$ (\method) & \textbf{68.20} & 78.46 & 66.12 & 69.23 & 63.40 & 67.36 & 63.41 & 70.31 & 69.82 & 63.97 & 65.89 & 65.25 & 74.06 & 67.03 & 67.78 & 71.81 \\
\bottomrule
\end{tabular}%
}
\caption{Performance of ToolSandbox on various scenarios and tool augmentations.
Our models are trained from \textbf{Qwen3-8B-Base}; we do not report results for the base checkpoint since it is not instruction-tuned under this evaluation protocol. Here, $\mathcal{D}_{\text{CS}}$ denotes the 8k cold-start SFT set, and $\mathcal{D}_{\text{RL}}$ denotes the 8k complex multi-turn, multi-step RL training set.}
\label{tab:scenario_tool_breakdown}
\end{table}

We evaluate our proposed \method using our final configuration (trajectory-level advantage estimation with group size $G=48$) on three challenging multi-turn, multi-step tool-use benchmarks: $\tau^2$-Bench, BFCL-V4, and ToolSandbox. We compare against the SFT counterparts and open-source models of similar size.

 
\paragraph{$\tau^2$-Bench Benchmark.}
The results on $\tau^2$-Bench are summarized in Table~\ref{tab:tau2_bench}.
% We follow the default evaluation setting of $\tau^2$-Bench. except that we retain the thinking content for our models to align with our training setup.
For each question, we run evaluation four times and report average accuracy. As shown in Table~\ref{tab:tau2_bench}, starting from \textbf{Qwen3-8B-Base}~\citep{qwen3technicalreport}, our RL model outperforms SFT by over 8 points, demonstrating the effectiveness of \method. 
However, our RL training uses a maximum context length of 10k and up to 30 turns, whereas $\tau^2$-Bench can require $>$30k context and up to 200 turns. Under this mismatch, \method lags behind some open-source models such as Qwen3-30B-A3B-Instruct-2507 and Qwen3-8B-Thinking.
To mitigate this, we further perform RL on an in-domain dataset, \textsc{APIGen}~\citep{}, which substantially improves average performance and surpasses the open-source baselines. Overall, these results indicate that \method is particularly effective when paired with in-domain data.


\paragraph{BFCL Benchmark.} 
Table~\ref{tab:bfcl_results} summarizes the results on BFCL-V4 (Multi-Turn and Web Search).
Overall, our RL model trained on $\mathcal{D}_{\text{RL}}$ (\method) substantially improves over SFT variants: on Multi-Turn, it achieves 36.50 overall accuracy, outperforming cold-start SFT and further SFT on $\mathcal{D}_{\text{RL}}$ by 10 points. 
On Web Search, RL also yields the best overall performance, improving over cold-start SFT and SFT on $\mathcal{D}_{\text{RL}}$ by 13.5 and 14 points, respectively.
Compared with open-source baselines, our RL model performs better than Qwen3-30B-A3B-Instruct-2507 (judging model) on Multi-Turn and is comparable to Qwen3-8B-Thinking, while significantly surpassing both baselines on Web Search.


\paragraph{ToolSandbox Benchmark.}
Table~\ref{tab:scenario_tool_breakdown} reports performance on ToolSandbox Benchmark.
RL on $\mathcal{D}_{\text{RL}}$ (\method) yields a large improvement over both SFT variants, increasing the overall score by more than 12 points.
It also improves consistently across nearly all scenario categories, with particularly notable gains on multi-turn and multi-tool settings.
Our RL model (\method) also outperforms the open-source models, including the judging model.


\paragraph{Summary.}
Our method consistently yields substantial gains over SFT, with improvements that are stable across benchmarks. Notably, the resulting policy matches and often surpasses the LLM-as-a-judge model on most evaluation measures, while remaining competitive with or exceeding similarly sized open-source baselines. We further find that a lightweight judge is sufficient to drive strong RL improvements, and the learned behavior generalizes well to previously unseen benchmarks.

% Moreover, incorporating in-domain RL data further strengthens performance, indicating that \method scales well with domain-aligned complex trajectories and provides a reliable recipe for improving multi-turn muti-step tool-use capabilities.

% \paragraph{Discussion: Scaling Up.}
% There are several natural axes to scale up \method. First, we can increase the \emph{number of checklist items per turn}, making the criteria denser and improving coverage of complex behaviors. Second, we can reduce residual judge noise by using \emph{majority voting} (or other ensembling schemes) over multiple independent judgments for the same checklist, trading extra compute for lower-variance rewards. Third, \method can benefit from \emph{stronger judge models}, which provide more reliable evidence grounding and more consistent binary decisions. Beyond checklist-specific knobs, standard scaling strategies also apply, including using a \emph{stronger base model} and a \emph{larger group size} for advantage estimation, both of which typically improve optimization stability.
% We expect these scaling directions to further stabilize training by suppressing residual stochasticity in tool use and judging. With sufficiently low-noise rewards, finer-grained reward assignment (e.g., step-level) may become viable, potentially retaining its fast early learning while avoiding premature collapse.


==> sec_arxiv/6_case_study.tex <==
\section{Case Study}

